Utilizing Dependencies to Obtain Subsets of Reachable Sets

Reachability analysis, in general, is a fundamental method that supports formally-correct synthesis, robust model predictive control, set-based observers, fault detection, invariant computation, and conformance checking, to name but a few. In many of these applications, one requires to compute a reachable set starting within a previously computed reachable set. While it was previously required to re-compute the entire reachable set, we demonstrate that one can leverage the dependencies of states within the previously computed set. As a result, we almost instantly obtain an over-approximative subset of a previously computed reachable set by evaluating analytical maps. The advantages of our novel method are demonstrated for falsification of systems, optimization over reachable sets, and synthesizing safe maneuver automata. In all of these applications, the computation time is reduced significantly.

==> Content.tex <==
% INTRODUCTION ---------------------------------------------

\section{Introduction}
\label{sec:Introduction}

Efficient set representations are highly relevant for controller synthesis and formal verification of hybrid systems, since many underlying algorithms compute with sets; see e.g., \cite{Bravo2006, Zamani2012, Kaynama2012, Schuermann2017c}. Improvements originating from a new set representation often significantly reduce computation time and improve the accuracy of set-based computations.


\paragraph{State of the Art}

\begin{figure}
\begin{center}
	\setlength{\belowcaptionskip}{-30pt}
	\includegraphics[width = 0.45 \textwidth]{figures/RelationsSetRepresentations.pdf}
	\caption{Visualization of the relations between the different set representations, where A $\rightarrow$ B denotes that B is a generalization of A.}
	\label{fig:RelationsSetRepresentations}
	\end{center}
\end{figure}

Fig. \ref{fig:RelationsSetRepresentations} shows relevant set representations and their relations to each other. Almost all typical set representations are convex, except Taylor models, star sets, and polynomial zonotopes. Since all convex sets can be represented by support functions, which are closed under Minkowski addition, linear maps, and convex hull operations, they are a good choice for reachability analysis \cite{Girard2008b,Frehse2011,Frehse2015,Schupp2017}. Ellipsoids and polytopes are special cases of support functions, which are often used for reachability analysis \cite{Chutinan2003,Kurzhanskiy2007,Schupp2017} and computations of invariant sets \cite{Blanchini1999,Alamo2005,Rungger2017,Legat2018}. However, the disadvantage of ellipsoids is that they are not closed under intersection and Minkowski addition; the disadvantage of polytopes is that Minkowski sum is computationally expensive \cite{Tiwary2008}. 

One important subclass of polytopes is zonotopes, which can be represented compactly by so-called generators: a zonotope with $m$ generators in $n$ dimensions might have up to ${m\choose n-1}$ halfspaces. More importantly, Minkowski sum and linear maps can be computed cheaply, making them a good choice for reachability analysis \cite{Girard2005,Althoff2014a,Althoff2016c}. Two relevant extensions to zonotopes are zonotope bundles \cite{Althoff2011f}, where the set is represented implicitly by the intersection of several zonotopes, and constrained zonotopes \cite{Scott2016}, where additional equality constraints on the zonotope factors are considered. Zonotope bundles, as well as constrained zonotopes, are both able to represent any polytope. Both representations make use of lazy computations and thus suffer much less from the curse of dimensionality as it is the case for polytopes \cite{Tiwary2008}. A special case of zonotopes are multi-dimensional intervals, which are particularly useful for range bounding of nonlinear functions via interval arithmetic \cite{Jaulin2006}, but they are also used for reachability analysis \cite{Eggers2012,Ramdani2011b}. Since intervals are not closed under linear maps, one often has to split them to reduce the wrapping effect \cite{Lohner2001}.

In general, reachable sets of nonlinear systems are non-convex, so that tight enclosures can only be achieved using non-convex set representations when avoiding splitting of reachable sets. Taylor models \cite{Makino2003}, which consist of a polynomial and an interval remainder part, are an example of non-convex set representation. They are typically used for range bounding \cite{Makino2005} and reachability analysis \cite{Chen2012}. Another type of non-convex set representation is polynomial zonotopes, which are introduced in \cite{Althoff2013a} and are a generalization of Taylor models as later shown in this work. Yet another way to represent non-convex sets is star sets, which are especially useful for simulation-based reachability analysis \cite{Duggirala2016,Bak2017}. While star sets are very expressive, it is yet unclear how some operations, such as nonlinear mapping, are computed. 

\paragraph{Overview}

In this work, we introduce a new non-convex set representation called \textit{sparse polynomial zonotopes}, which is a non-trivial extension of polynomial zonotopes from \cite{Althoff2013a} and exhibits the following major advantages: a) sparse polynomial zonotopes enable a very compact representation of sets, b) they are closed under all relevant operations, c) many other set representations can be converted to an sparse polynomial zonotope, and most important, d) all operations have at most polynomial complexity.

The remainder of this paper is structured as follows: In Sec. \ref{sec:SparsePolynomialZonotope}, the formal definition of sparse polynomial zonotopes is provided and important operations on them are derived. We show how sparse polynomial zonotopes provide substantially better results for reachability analysis in Sec. \ref{sec:ReachabilityAnalysis}, which is demonstrated in Sec. \ref{sec:NumericalExamples} on two numerical examples. 


\paragraph{Notation}

In the remainder of this paper, we will use the following notations: Sets are always denoted by calligraphic letters, matrices by uppercase letters, and vectors by lowercase letters. Given a discrete set $\mathcal{H} \in \{ \cdot \}^n$, $|\mathcal{H}| = n$ denotes the cardinality of the set and $\mathcal{H}_{(i)}$ refers to the $i$-th entry of the set $\mathcal{H}$. Given a vector $b \in \mathbb{R}^n$, $b_{(i)}$ refers to the $i$-th entry. Given a matrix $A \in \mathbb{R}^{n \times m}$, $A_{(i,\cdot)}$ represents the $i$-th matrix row, $A_{(\cdot,j)}$ the $j$-th column, and $A_{(i,j)}$ the $j$-th entry of matrix row $i$. Given a discrete set of positive integer indices $\mathcal{H}$ with $|\mathcal{H}| < m$, $A_{(\cdot,\mathcal{H})}$ is used for $[ A_{\left( \cdot, \mathcal{H}_{(1)} \right)} ~ \dots ~ A_{\left( \cdot, \mathcal{H}_{(|\mathcal{H}|)} \right)} ]$, where $[C~D]$ denotes the concatenation of two matrices $C$ and $D$. The symbols $\mathbf{0}$ and $\mathbf{1}$ represent matrices of zeros and ones of proper dimension. The left multiplication of a matrix $M \in \mathbb{R}^{m \times n}$ with a set $\mathcal{S} \subset \mathbb{R}^n$ is defined as $M \otimes \mathcal{S} = \{ M \cdot s ~ | ~ s \in \mathcal{S} \}$, and the Minkowski addition of two sets $\mathcal{S}_1 \subset \mathbb{R}^n$ and $\mathcal{S}_2 \subset \mathbb{R}^n$ is defined as $\mathcal{S}_1 \oplus \mathcal{S}_2 = \{ s_1 + s_2 ~|~ s_1 \in \mathcal{S}_1, s_2 \in \mathcal{S}_2 \}$. We further introduce an n-dimensional interval as $\mathcal{I} := [l,u],~ \forall i ~ l_{(i)} \leq u_{(i)},~ l,u \in \mathbb{R}^n$. For the derivation of computational complexity, we consider all binary operations exept concatenations, and initializations are explicitly not considered. 





% SPARSE POLYNOMIAL ZONOTOPES ------------------------------

\section{Sparse Polynomial Zonotopes} 
\label{sec:SparsePolynomialZonotope}

Let us first define sparse polynomial zonotopes (\SPZs), followed by derivations of relevant operations on them. 
\begin{definition}
  Given a generator matrix of dependent generators $G \in \mathbb{R}^{n \times h}$, a generator matrix of independent generators $G_I \in \mathbb{R}^{n \times q}$, and an exponent matrix $E \in \mathbb{Z}_{\ge 0}^{p \times h}$, an \SPZl is defined as  
  \begin{equation}
  	\begin{split}
    \mathcal{PZ} = \bigg\{ & \left. \sum _{i=1}^h \left( \prod _{k=1}^p \alpha _k ^{E_{(k,i)}} \right) G_{(\cdot,i)} + \sum _{j=1}^{q} \beta _j G_{I(\cdot,j)} \right| \\ & \alpha_i, \beta_j \in [-1,1] \bigg\}.
    \end{split}
  \label{eq:polyZonotope}
  \end{equation}
\end{definition}  
The scalars $\alpha_i$ are called \textit{ dependent factors} since a change in their value affects multiplication with multiple generators. Consequently, the scalars $\beta_j$ are called \textit{independent factors} because they only affect multiplication with one generator. The number of dependent factors is $p$, the number of independent factors is $q$, and the number of dependent generators is $h$. The order of an \SPZl $\rho$ is defined as $\rho = \frac{h + q}{n}$. For the derivation of the computational complexity of set operations, we introduce 
\begin{equation}
	h = c_h n, ~ p = c_p n ,~ q = c_q n,
	\label{eq:complexity}
\end{equation} 
with $c_h,c_p,c_q \in \mathbb{R}_{\geq 0}$. In the remainder of this paper, we call the single term $\alpha_1^{E_{(1,i)}} \cdot \dotsc \cdot \alpha_p^{E_{(p,i)}} \cdot G_{(\cdot,i)}$ a monomial, and $\alpha_1^{E_{(1,i)}} \cdot \dotsc \cdot \alpha_p^{E_{(p,i)}}$ the variable part of the monomial. In order to keep track of the dependencies between the dependent factors from different \SPZs, we introduce an unambiguous integer identifier for each dependent factor $\alpha_i$ and store the identifiers for all dependent factors in a list $\mathcal{ID} \in \{\mathbb{N}\}^p$. Using this identifier list, we introduce the shorthand $\mathcal{PZ} = \left\{ G, G_I, E, \mathcal{ID} \right\} \subset \mathbb{R}^n$ for the representation of \SPZs.
All components of a set $\square_i$ have the index $i$, e.g., $p_i$, $h_i$, and $q_i$ belong to $\mathcal{PZ}_i$. To make \SPZsl more intuitive, we introduce the following example:

\begin{example} 
	The \SPZl
	\begin{equation}
		\mathcal{PZ} = \left\{ \begin{bmatrix} 2 & 1 & 2 \\ 0 & 2 & 2 \end{bmatrix}, \begin{bmatrix} 1 \\ 0 \end{bmatrix}, \begin{bmatrix} 1 & 0 & 3 \\ 0 & 1 & 1 \end{bmatrix}, \{ 1, 2 \} \right\},
	\label{eq:Example}
	\end{equation}
	defines the set
	\begin{equation}
	\begin{split}
  		\mathcal{PZ} = \bigg\{ & \begin{bmatrix} 2 \\ 0 	\end{bmatrix} \alpha_1 + \begin{bmatrix} 1 \\ 2 \end{bmatrix} \alpha_2 + \begin{bmatrix} 2 \\ 2 \end{bmatrix} \alpha_1^3 \cdot \alpha_2 + \begin{bmatrix} 1 \\ 0 \end{bmatrix} \beta_1 \bigg| \\ & \alpha_1, \alpha_2, \beta_1 \in [-1,1] \bigg\}.
	\end{split}
	\end{equation}
	\label{ex:PolyZonotope}
\end{example}
The construction of this \SPZl is visualized in Fig. \ref{fig:Example}: (a) shows the set spanned by the first two dependent generators, (b) shows the addition of the dependent generator with the mixed term $\alpha_1^3 \cdot \alpha_2$, (c) shows the addition of the independent generator, and (d) visualizes the final set. 

\begin{figure}
\begin{center}
	\setlength{\belowcaptionskip}{-10pt}
	\includegraphics[width = 0.45 \textwidth]{figures/polyZonotopeExample.pdf}
	\caption{Construction of the \SPZl in Example \ref{ex:PolyZonotope} from the single generator vectors.}
	\label{fig:Example}
	\end{center}
\end{figure}

Our sparse representation is a non-trivial extension of polynomial zonotopes \cite[Def. 1]{Althoff2013a}, resulting in completely different algorithms for operations on them. In \cite{Althoff2013a}, the generators for all possible combinations of dependent factors up to a certain polynomial degree are stored. For the one-dimensional polynomial zonotope $\mathcal{PZ} = \{ \alpha_1 \cdot \ldots \cdot \alpha_{19} \cdot \alpha_{20}^{10} | \alpha_i \in [-1,1] \}$ with $p=20$ dependent factors and with a polynomial degree of $10$, the number of dependent generators is $h = 30045015$. This demonstrates that the number of stored generators can become very large if the polynomial degree and the number of dependent factors are high, which makes computations on the previous set representation very inefficient. We in turn use a sparse representation, where only the generators for desired factor combinations are stored, which enables the representation of the above polynomial zonotope with only one single generator. Furthermore, our representation does not require limiting the polynomial degree of the polynomial zonotope in advance, which is advantageous for reachability analysis, as shown in Sec. \ref{subsec:advantages}.  


% Preliminary operations

\subsection{Preliminary Operations}

First, we introduce preliminary set operations that are required for many other operations.

% Merge of set identifiers

\paragraph{Merging the Set of Identifiers}

For all set operations that involve two or more \SPZs, the operator $mergeID()$ is necessary in order to build a common representation of exponent matrices to fully exploit the dependencies between identical dependent factors:

\begin{proposition}
	(Merge ID) Given two \SPZs, $\mathcal{PZ}_1 = \{G_1,\linebreak[1] G_{I,1}, E_1, \mathcal{ID}_1 \}$ and $\mathcal{PZ}_2 = \{G_2, \linebreak[1] G_{I,2},$ $E_2, \mathcal{ID}_2 \}$, \lword{$mergeID()$} returns two adjusted \SPZsl with identical identifier lists that are equivalent to $\mathcal{PZ}_1$ and $\mathcal{PZ}_2$, and has a complexity of $\mathcal{O}(n^2)$:
	\begin{displaymath}
	\begin{split}
		& mergeID(\mathcal{PZ}_1,\mathcal{PZ}_2) = \big \{ \{ G_1, G_{I,1}, \overline{E}_1, \overline{\mathcal{ID}} \}, \\
		& ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ \{ G_2, G_{I,2}, \overline{E}_2, \overline{\mathcal{ID}} \}\big \} \\
		& with ~~ \overline{\mathcal{ID}} = \left\{\mathcal{ID}_1, \mathcal{ID}_{2(\mathcal{H}_{(1)})}, \dots , \mathcal{ID}_{2 (\mathcal{H}_{(|\mathcal{H}|)})} \right\} \\
		& ~~~~~~~ \overline{E}_1 = \begin{bmatrix} E_1 \\ \mathbf{0} \end{bmatrix} \in \mathbb{R}^{a \times h_1} \\
		& ~~~~~~~ \overline{E}_{2(i,\cdot)} = \begin{cases} E_{2(j,\cdot)},~ if ~ \exists j~\overline{\mathcal{ID}}_{(i)} = \mathcal{ID}_{2(j)} \\ \mathbf{0}~, ~~~~~~ else \end{cases} i = 1 \dots a \\
		& ~~~~~~~ \mathcal{H} = \left\{ i~ |~ \mathcal{ID}_{2(i)} \not\in \mathcal{ID}_1 \right\},
	\end{split}
	\end{displaymath}
where $a = |\mathcal{H}|+p_1$.
\end{proposition}

\begin{proof}
	(Merge ID) The extension of the exponent matrices with all-zero rows only changes the representation of the set, but not the set itself.
	
Complexity:	The only operation with super-linear complexity is the construction of the set $\mathcal{H}$ with $\mathcal{O}(p_1 \cdot p_2) = \mathcal{O}(n^2)$ using \eqref{eq:complexity}.
\end{proof}


% Transformation to a minimal representation

\paragraph{Transformation to a Compressed Representation}

Some set operations result in an \SPZl that contains multiple monomials with an identical variable part, which we combine to one single monomial:

\begin{proposition}
	(Compact) Given an \SPZl $\mathcal{PZ} = \{G,G_I,\linebreak[0]E,\mathcal{ID} \}$, the operation $compact()$ returns a compressed representation of the set $\mathcal{PZ}$ and has a complexity of $\mathcal{O}(n^2 \log (n))$:
	\begin{equation}
		\begin{split}
			& compact(\mathcal{PZ}) = \{ \overline{G}, G_I, \overline{E}, \mathcal{ID} \} \\
			& with ~~ \overline{E} = uniqueColumns( E ) \in \mathbb{Z}_{\ge 0}^{p \times k} \\
			& ~~~~~~~~ \mathcal{M}_j = \big \{ i~ |~ \overline{E}_{(l,j)} = E_{(l,i)} ~ \forall l \in \{1 \dots p\} \big \} \\
			& ~~~~~~~~ \overline{G} = \bigg[ \sum_{i \in \mathcal{M}_1} G_{(\cdot,i)} ~ \dots ~ \sum_{i \in \mathcal{M}_k} G_{(\cdot,i)} \bigg],
		\end{split}
	\end{equation}
	where the operation $uniqueColumns()$ removes identical matrix columns until all columns are unique.
\end{proposition}

\begin{proof}
	(Compact) Since the number of unique columns $k$ of matrix $E$ is smaller than the number of overall columns $h$, the matrices $\overline{E}$ and $\overline{G}$ are smaller or of equal size compared to the matrices $E$ and $G$, which results in a compressed representation of the set. 
	
Complexity:	The operation $uniqueColumns()$ in combination with the construction of the sets $\mathcal{M}_j$ can be efficiently implemented by sorting the matrix columns followed by an identification of identical neighbors, which can be realized with a worst case complexity of $\mathcal{O}(p h \log (h))$. Since all other operations have at most quadratic complexity, the overall complexity is $\mathcal{O}(n^2 \log (n))$ using \eqref{eq:complexity}.
\end{proof}
The operation $compact()$ is applied after all set operations that potentially result in \SPZsl containing multiple monomials with identical variable part. These operations are conversion from a Taylor model, Minkowski addition and quadratic map. 



% Conversion from other set representations

\subsection{Conversion from other Set Representations}

This section shows how other set representations can be converted to \SPZs.


% Zonotope

\paragraph{Zonotope and Interval}

We first provide the definition of a zonotope:

\begin{definition}
	(Zonotope) \cite[Def. 1]{Girard2005} Given a center $c \in \mathbb{R}^n$ and a generator matrix $G \in \mathbb{R}^{n \times m}$, a zonotope is defined as 
	\begin{equation}
		\mathcal{Z} = \left\{ \left. c + \sum_{i=1}^m \alpha_i G_{(\cdot,i)} ~\right|~ \alpha_i \in [-1,1] \right\}.
	\label{eq:zonotope}
	\end{equation}
\end{definition}

For a compact notation, we introduce the shorthand $\mathcal{Z} = \{c,G \}$. Any zonotope can be converted to an \SPZ:

\begin{proposition}
	(Conversion Zonotope) A zonotope $\mathcal{Z} = \{c, G \}$ can be represented by an \SPZl $\mathcal{PZ}$:
	\begin{equation}
		\mathcal{PZ} = \left\{ [c ~ G] ,\mathbf{0},[\mathbf{0} ~ I],\{1,...,m\} \right\},
	\end{equation}
	where $I \in \mathbb{R}^{m \times m}$ is the identity matrix. The complexity of the conversion is $\mathcal{O}(1)$.
	\label{prop:conversionZonotope}
\end{proposition}

\begin{proof}
	(Conversion Zonotope) If we insert $E = [\mathbf{0} ~ I]$ and $G_I = \mathbf{0}$ into \eqref{eq:polyZonotope}, we obtain a zonotope (see \eqref{eq:zonotope}). 
	
Complexity:	The complexity is constant since the conversion only involves concatenations and initializations.
\end{proof}
Since any interval can be represented as a zonotope \cite[Prop. 2.1]{Althoff2010a}, their conversion to an \SPZl is straightforward.




% Taylor model

\paragraph{Taylor Model}

First, we formally define multi-dimensional Taylor models:

\begin{definition}
	(Taylor Model) \cite[Def. 2.1]{Chen2012} Given a vector field $p: \mathbb{R}^n \to \mathbb{R}^n$, where each subfunction $p_{(i)}: \mathbb{R}^n \to \mathbb{R}$ is a polynomial function defined as  
	\begin{equation}
		p_{(i)} \left( x_{(1)},\dots ,x_{(n)} \right) = \sum_{j = 1}^{m_i} b_{i(j)} \prod_{k=1}^n	x_{(k)}^{E_{i(k,j)}},
		\label{eq:polyFuncTaylorModel}	
	\end{equation}
	and an interval $\mathcal{I} \subset \mathbb{R}^n$, a Taylor model $\mathcal{T}(x) \subset \mathbb{R}^n$ is defined as 
	\begin{equation}
		\mathcal{T}(x) = \left\{ \left. \begin{bmatrix} p_{(1)}(x) \\ \vdots \\ p_{(n)}(x) \end{bmatrix} + \begin{bmatrix} y_{(1)} \\ \vdots \\ y_{(n)} \end{bmatrix} ~ \right| ~ y \in \mathcal{I} \right\},
	\end{equation}
	where $E_i \in \mathbb{Z}_{\ge 0}^{n \times m_i}$ represents an exponent matrix and $b_i \in \mathbb{R}^{m_i}$ is a vector of polynomial coefficients. 
\end{definition}
For a concise notation, we introduce the shorthand $\mathcal{T}(x) = \{ p, \mathcal{I} \}$. The set defined by any Taylor model can be converted to an \SPZ:

\begin{theorem}
	(Conversion Taylor Model) The set defined by a Taylor model $\mathcal{T}(x) = \{ p, \mathcal{I} \}$ on the domain $x \in \mathcal{D}$ with $\mathcal{D} = [l_d,u_d]$ and $\mathcal{I} = [l_r,u_r]$ can be equivalently represented by an \SPZl $\mathcal{PZ}$:
	\begin{equation}
		\begin{split}
			& \mathcal{PZ} = \left\{ \left[ \frac{l_r + u_r}{2} ~ \hat{G} \right] , G_I, [ \mathbf{0} ~ \hat{E}], \{1,\dots ,n \} \right\} \\
			& with ~~ \hat{G} = \begin{bmatrix} \overline{b}_1^T &  & \mathbf{0} \\ & \ddots & \\ \mathbf{0} &  & \overline{b}_n^T \end{bmatrix}, \hat{E} = \begin{bmatrix} \overline{E}_1 \dots \overline{E}_n \end{bmatrix}, \\
			& ~~~~~~~~ G_I = \begin{bmatrix} \frac{u_{r(1)}-l_{r(1)}}{2} & & \mathbf{0} \\ & \ddots & \\ \mathbf{0} & & \frac{u_{r(n)}-l_{r(n)}}{2} \end{bmatrix}.
		\end{split}
		\label{eq:conversionTaylorModel}
	\end{equation}
	The vectors $\overline{b}_i$ and the matrices $\overline{E}_i$ result from the definition
	\begin{equation}
		p_{(i)} \left( \epsilon_1,\dots ,\epsilon_n \right) = \sum_{j = 1}^{\overline{m}_i} \overline{b}_{i(j)} \prod_{k=1}^n	\alpha_k^{\overline{E}_{i(k,j)}},
	\label{eq:TaylorModelTransform}
	\end{equation}
	where $\epsilon_k = 0.5 (l_{d(k)} + u_{d(k)}) + 0.5 \alpha_k (u_{d(k)} - l_{d(k)}),~\alpha_k \in [-1,1], ~k=1\dots n$, and $p_{(i)}(\cdot)$ is defined as in \eqref{eq:polyFuncTaylorModel}. The complexity of the conversion is $\mathcal{O}(n^5 ~ 2^{n^2})$.
\end{theorem}

\begin{proof}
	(Conversion Taylor model) The auxiliary variables $\epsilon_k$ represent the domain $\mathcal{D}$ with dependent factors $\alpha_k \in [-1,1]$. Evaluation of the polynomial functions $p_{(i)}(\cdot)$ from \eqref{eq:polyFuncTaylorModel} with the substitution $x_{(k)} = \epsilon_k$ in \eqref{eq:TaylorModelTransform} therefore directly yields the definition of the dependent part of an \SPZl (see \eqref{eq:polyZonotope}). The equation for the independent generator matrix $G_I$ follows from the representation of the interval $\mathcal{I}= [l_r,u_r]$ as a zonotope $\mathcal{Z} = \{0.5(l_r+u_r), 0.5 ~ diag(u_{r(1)}-l_{r(1)}, \dots, u_{r(n)}-l_{r(n)}  ) \}$, where the operator $diag()$ constructs a diagonal matrix. 
	
Complexity: Let $m = \max (m_1,\dots,m_n)$ and $e = \max ( \linebreak[1] \max(E_1), \dots , \max(E_n))$, where $\max (A)$ returns the maximum entry of matrix $A$. The exponent matrix $\hat{E}$ has $\hat{h} = n m (2^e)^n$ columns in the worst case, resulting from the evaluation of the functions $p_{(i)} \left( \epsilon_1,\dots ,\epsilon_n \right)$. Since the complexity of $compact()$ is $\mathcal{O}(\hat{p} \hat{h} \log(\hat{h}))$ and $\hat{p} = n$, the subsequent application of the $compact()$ operation has complexity $\mathcal{O}(n^2 m (2^e)^n \log(n m (2^e)^n)) = \mathcal{O}(n^2 m ~ 2^{en}(\log(n) + \log(m) + ne \log(2))) = \mathcal{O}(n^5 ~ 2^{n^2})$ using \eqref{eq:complexity}. This is also the overall complexity of the conversion, since all other operations have a lower complexity. 
\end{proof}

\begin{corollary}
	The set defined by any Taylor model can be equivalently represented by an \SPZ, but not every \SPZl can be represented by a Taylor model.
\end{corollary}
The corollary follows directly from the fact that the number of dependent factors $p$ of an \SPZl can be larger than the dimension of the state space $n$, which includes the special case of Taylor models for which $p$ equals $n$. 







% Over-Approximation

\subsection{Enclosure by other Set Representations}

This subsection describes how \SPZsl can be enclosed by other set representations. 

% Zonotope

\paragraph{Zonotope}

We first show how an \SPZl can be enclosed by a zonotope:

\begin{proposition}
	(Zonotope) Given an \SPZl $\mathcal{PZ} = \{ G,G_I,\linebreak[1] E,\mathcal{ID} \}$, the operation $zono()$ returns a zonotope that encloses $\mathcal{PZ}$ and has a complexity of $\mathcal{O}(n^2)$:
	\begin{equation}
		\begin{split}
			& zono\left( \mathcal{PZ} \right) = \bigg\{ \sum_{j=1}^{|\mathcal{N}|} G_{\left(\cdot, \mathcal{N}_{(j)} \right) } + \frac{1}{2} \sum_{i=1}^{|\mathcal{H}|} G_{\left(\cdot, \mathcal{H}_{(i)} \right)}, \\
			& ~~~~~~~~~~~~~~~~~~ \begin{bmatrix} \frac{1}{2} G_{(\cdot,\mathcal{H})} & G_{(\cdot,\mathcal{K})} & G_I\end{bmatrix} \bigg\} \\
			& with ~~ \mathcal{N} = \left\{ i ~ \left|~ E_{(j,i)} = 0 ~ \forall j \in \{ 1 \dots p \} \right. \right\} \\
			& ~~~~~~~~ \mathcal{H} = \left\{ i ~\left|~ \prod_{j=1}^p \left(1-(E_{(j,i)} \mathrm{mod} ~ 2)\right) = 1 \right. \right\} \setminus \mathcal{N} \\
			& ~~~~~~~~ \mathcal{K} = \{1, \dots ,h\} \setminus ( \mathcal{H} \cup \mathcal{N} ).
		\end{split}
	\end{equation}
\end{proposition}

\begin{proof}
	(Zonotope) The over-approximation of all monomial variable parts in \eqref{eq:polyZonotope} with additional independent factors removes the dependence between the dependent factors and yields the definition of a zonotope \eqref{eq:zonotope}. This zonotope encloses $\mathcal{PZ}$ because removing dependence results in an over-approximation \cite{Jaulin2006}. Since monomials with exclusively even exponents ($i \in \mathcal{H}$) are strictly positive, we can enclose them tighter using
	\begin{equation}
		\begin{split}
			\forall i \in \mathcal{H}: ~~ & \left( \prod_{k=1}^p [-1,1]^{E_{(k,i)}} \right) G_{(\cdot, i)} = [0,1] G_{(\cdot, i)} = \\ & ~~~~~~ = \frac{1}{2} G_{(\cdot, i)} + [-1,1] \frac{1}{2} G_{(\cdot, i)}.
		\end{split}
	\end{equation}
	For all other monomials, evaluation of the monomial variable part directly results in the interval $[-1,1]$. 
	
Complexity:	The calculation of the set $\mathcal{H}$ has complexity $\mathcal{O}(ph)$, and the construction of the zonotope $\mathcal{O}(nh)$ in the worst case, resulting in an overall complexity of $\mathcal{O}(ph) + \mathcal{O}(nh)$, which is equal to $\mathcal{O}(n^2)$ using \eqref{eq:complexity}. 
\end{proof}





% Support Function, Interval and Template Polyhedra

\paragraph{Support Function, Interval, and Template Polyhedra}

Let us first derive the support function of an \SPZ.

\begin{definition}
	(Support Function) \cite[Def. 1]{Girard2008b} Given a set $\mathcal{S} \subset{R}^n$ and a direction $d \in \mathbb{R}^n$, the support function $s_{\mathcal{S}}: \mathbb{R}^n \to \mathbb{R}$ of $\mathcal{S}$ is defined as 
	\begin{equation}
		s_{\mathcal{S}}(d) = \max\limits_{x \in \mathcal{S}} ~ d^T x.
	\end{equation} 
\end{definition}
If $\mathcal{S}$ is convex, its support function is an exact representation; otherwise, an over-approximation is returned. Since \SPZsl are non-convex in general, one can only over-approxi\-mate them by support functions. 

\begin{proposition}
	(Support Function) Given an \SPZl $\mathcal{PZ} = \{ G,G_I,E,\mathcal{ID} \}$ and a direction $d \in \mathbb{R}^n$, the support function $\hat{s}_{\mathcal{PZ}}(d)$ over-approximates $\mathcal{PZ}$:
	\begin{equation}
		\begin{split}
			& \hat{s}_{\mathcal{PZ}}(d) = u + \sum_{j=1}^q \left| \overline{g}_{I(j)} \right| \\
			& with ~~ [l,u] = B\left(w(\alpha_1, \dots , \alpha_{p}),[-\mathbf{1},\mathbf{1}]\right),
		\end{split}
		\label{eq:supportFunction} 
	\end{equation}
where $d^T \otimes \mathcal{PZ}= \linebreak[1] \{ \overline{g}, \linebreak[1] \overline{g}_I, \linebreak[1] E, \linebreak[1] \mathcal{ID} \}$ is the projection of $\mathcal{PZ}$ onto the vector $d$. The polynomial function $w: \mathbb{R}^{p} \to \mathbb{R}$ is defined by the dependent generators as
\begin{equation}
	w(\alpha_1, \dots , \alpha_{p}) = \sum _{i=1}^{h} \left( \prod _{k=1}^{p} \alpha _k ^{E_{(k,i)}} \right) \overline{g}_{(i)}.
\label{eq:polyFunc}
\end{equation}
Furthermore, given a function $f: \mathbb{R}^{m} \to \mathbb{R}$ and an interval $\mathcal{I} \subset \mathbb{R}^m$, the range bounding operation
	\begin{equation}
		B(f(x),\mathcal{I}) = \left[\min\limits_{x \in \mathcal{I}} f(x),~ \max\limits_{x \in \mathcal{I}} f(x)\right]
	\end{equation}
returns an over-approximation of the exact bounds. The calculation of $\hat{s}_{\mathcal{PZ}}(d)$ has complexity $\mathcal{O}(n^2) + \mathcal{O}(B())$, where $\mathcal{O}(B())$ denotes the computational complexity of the range bounding operation.
\label{prop:bound}
\end{proposition}  

\begin{proof}
	(Support Function) We first project the \SPZl onto the vector $d$, and then split the one-dimensional projected \SPZl into one part with independent generators and one with dependent generators: The bounds for the independent part calculated by the sum of absolute values in \eqref{eq:supportFunction} are exact \cite[Sec. 2]{Girard2008b}. However, the upper bound $u$ of the dependent part in \eqref{eq:supportFunction} is over-approximative since the range bounding operation $B()$ returns an over-approximation, so that $\hat{s}_{\mathcal{PZ}}(d)$ over-approximates $\mathcal{PZ}$. 

Complexity: The calculation of the projection onto $d$ has a complexity of $\mathcal{O}(nh) + \mathcal{O}(nq)$ (see Sec. \ref{sec:basicSetOperations}), which results in an overall complexity of $\mathcal{O}(n^2) + \mathcal{O}(B())$ using \eqref{eq:complexity} since all other operations have linear complexity. 
\end{proof}
Note that the tightness of $\hat{s}_{\mathcal{PZ}}(d)$ solely depends on the tightness of the bounds of the function $w(\cdot)$ obtained by one of the range bounding techniques, e.g., interval arithmetic \cite{Jaulin2006} and verified global optimization \cite{Makino2005}. %A comparision of different techniques can be found in \cite{Althoff2018}. 

A template polyhedron enclosing an \SPZl can easily be constructed by evaluating the support function $\hat{s}_\mathcal{PZ}(d)$ for a discrete set of directions $\mathcal{D} = \{d_1, \dots , d_w \}$. The over-approximation with an interval represents a special case where $\mathcal{D} = \{ I_{(\cdot,1)}, \linebreak[1] \dots, \linebreak[1] I_{(\cdot,n)},\linebreak[1] -I_{(\cdot,1)},\linebreak[1] \dots, \linebreak[1] -I_{(\cdot,n)} \}$ with $I \in \mathbb{R}^{n \times n}$ being the identity matrix. 






% Basic set operations

\subsection{Basic Set Operations}
\label{sec:basicSetOperations}

This subsection derives basic operations on \SPZs.



% Multiplication with matrix

\paragraph{Multiplication with a Matrix}

The left-multiplication with a matrix is obtained as:

\begin{proposition}
	(Multiplication) Given an \SPZl $\mathcal{PZ} = \{ G, \linebreak[1] G_I,E,\mathcal{ID} \} \subset \mathbb{R}^n$ and a numerical matrix $M \in \mathbb{R}^{m \times n}$, the left-multiplication is computed as 
	\begin{equation}
		M \otimes \mathcal{PZ} = \left\{ MG, MG_I, E, \mathcal{ID} \right\},
	\end{equation}
	which has complexity $\mathcal{O}(mn^2)$.
\end{proposition}

\begin{proof}
	(Multiplication) The result follows directly from inserting the definition of \SPZsl in \eqref{eq:polyZonotope} into the definition of the operator $\otimes$ (see \textit{Notation} in Sec. \ref{sec:Introduction}). 
	
Complexity: The complexity results from the complexity of matrix multiplications and is therefore $\mathcal{O}(mnh) + \mathcal{O}(mnq) = \mathcal{O}(mn^2)$ using \eqref{eq:complexity}.
\end{proof}



% Minkowski Sum

\paragraph{Minkowski Addition}

Even though every zonotope can be represented as an \SPZ, we provide a separate definition for the Minkowski addition of an \SPZl and a zonotope for computational reasons. If two \SPZsl are involved, we first have to bring the exponent matrices to a common representation using $mergeID()$.
\begin{proposition}
	(Addition) Given two \SPZs, $\mathcal{PZ}_1 = \{G_1, \linebreak[1] G_{I,1}, E_1, \mathcal{ID}_1 \}$ and $\mathcal{PZ}_2 = \{G_2, G_{I,2},$ $E_2, \mathcal{ID}_2 \}$, as well as a zonotope $\mathcal{Z} = \{ c_z,G_z \}$, their Minkowski sum is defined as
	\begin{equation}
		\begin{split}
			\mathcal{PZ}_1 \oplus \mathcal{PZ}_2 = \big\{ & \begin{bmatrix} G_1 & G_2 \end{bmatrix}, \begin{bmatrix} G_{I,1} & G_{I,2} \end{bmatrix}, \\ & \begin{bmatrix} E_1 & E_2 \end{bmatrix} , \mathcal{ID}_1 \big\},
		\end{split}
		\label{eq:addition}
	\end{equation}	
	\begin{equation}
		\mathcal{PZ}_1 \oplus \mathcal{Z} = \big\{ \begin{bmatrix} c_z & G_1 \end{bmatrix}, \begin{bmatrix} G_{I,1} & G_z \end{bmatrix}, \begin{bmatrix} \mathbf{0} & E_1 \end{bmatrix}, \mathcal{ID}_1 \big\},
		\label{eq:additionZonotope}
	\end{equation}
	where \eqref{eq:addition} has complexity $\mathcal{O}(n^2 \log(n))$ and \eqref{eq:additionZonotope} has complexity $\mathcal{O}(1)$.  
	\label{prop:addition}
\end{proposition}
\begin{proof}
	(Addition) Since the operation $mergeID()$ is applied beforehand, $\mathcal{ID}_1 = \mathcal{ID}_2$. The result is obtained by inserting the definition of zonotopes \eqref{eq:zonotope} and \SPZsl \eqref{eq:polyZonotope} into the definition of the Minkowski sum (see $Notation$ in Sec. \ref{sec:Introduction}). 

Complexity: The construction of the resulting \SPZsl only involves concatenations and therefore has complexity $\mathcal{O}(1)$. For two \SPZs, the $compact()$ operation with complexity $\mathcal{O}(p_1(h_1 + h_2) \log(h_1 + h_2))$ has to be additionally applied, resulting in an overall complexity of $\mathcal{O}(n^2 \log (n))$ using \eqref{eq:complexity}. 
\end{proof}




% Quadratic Map

\paragraph{Quadratic Map}

For reachability analysis based on the conservative polynomialization approach \cite{Althoff2013a}, a polynomial abstraction of the nonlinear dynamic function is calculated, requiring quadratic and higher order mappings. Here, we derive the equations for the quadratic map.

\begin{definition}
	(Quadratic Map) \cite[Theorem 1]{Althoff2013a} Given a set $\mathcal{S} \subset \mathbb{R}^n$ and a discrete set of matrices $Q_{i} \in \mathbb{R}^{n \times n}, i = 1 \dots m$, the quadratic map of $\mathcal{S}$ is defined as 
	\begin{equation}
		sq(Q,\mathcal{S}) = \left\{ x \left|~ x_{(i)} = s^T Q_{i} s,~ s \in \mathcal{S},~i = 1 \dots m \right. \right\}.
	\end{equation}
	\label{def:quadMap}
\end{definition}
For \SPZs, we first consider the special case without independent generators, and later present the general case.
 
\begin{proposition}
Given the \SPZl $\widehat{PZ} \linebreak[1] = \{ \hat{G},\mathbf{0}, \hat{E}, \widehat{\mathcal{ID}} \}$ and a discrete set of matrices $Q_{i} \in \mathbb{R}^{n \times n}, i = 1 \dots m$, the result of the quadratic map is
	\begin{equation}
		\begin{split}
		& sq(Q,\mathcal{\widehat{PZ}}) = \{\overline{G}, \mathbf{0}, \overline{E}, \widehat{\mathcal{ID}} \} \\
		& with ~~ \overline{E} = \big [ \hat{E}^{(1)} \dots ~ \hat{E}^{(\hat{h})} \big ],~ \overline{G} = \big [ \hat{G}^{(1)} \dots ~ \hat{G}^{(\hat{h})} \big ],
	\end{split}
	\label{eq:quadMap}
	\end{equation}
where 
	\begin{equation}
		\hat{E}^{(j)} = \hat{E} + \hat{E}_{(\cdot,j)} \cdot \mathbf{1} , ~~ \hat{G}^{(j)} = \begin{bmatrix} \hat{G}_{(\cdot,j)}^T Q_{1} \hat{G} \\ \vdots \\ \hat{G}_{(\cdot,j)}^T Q_{m} \hat{G} \end{bmatrix}.
	\end{equation}
	The overall complexity is $\mathcal{O}(n^3 m)$.
	\label{prop:quadMap1}
\end{proposition}

\begin{proof}
	The equations are obtained directly by substitution of $s$ in Def. \ref{def:quadMap} with the definition of an \SPZl from \eqref{eq:polyZonotope}, where we exploit that $\alpha^{e_1} \cdot \alpha^{e_2} = \alpha^{e_1+e_2}$ holds. 
	
Complexity: The construction of the matrices $\hat{E}^{(j)}$ has complexity $\mathcal{O}(\hat{h}^2 \hat{p})$, and the construction of the matrices $\hat{G}^{(j)}$ has complexity $\mathcal{O}(n^2 \hat{h} m) + \mathcal{O}(n \hat{h}^2 m)$ if the results for $Q_i \hat{G}$ are stored and reused. The resulting overall complexity is $\mathcal{O}(n^3 m)$ using \eqref{eq:complexity}.
\end{proof}
We now extend Prop. \ref{prop:quadMap1} to the general case including independent generators, for which we compute an over-approxi\-mation for computational reasons.

\begin{proposition}
	(Quadratic Map) Given an \SPZl $\mathcal{PZ} = \{ G,G_I,E,\mathcal{ID} \} \subset \mathbb{R}^n$ and a discrete set of matrices $Q_{i} \in \mathbb{R}^{n \times n}, i = 1 \dots m$,
	\begin{equation}
		sq(Q,\mathcal{PZ}) \subseteq \left\{ \big[ c_z ~ \overline{G}_{(\cdot,\mathcal{H})} \big], G_z, \big[ \mathbf{0} ~ \overline{E}_{\left(\{ 1 \dots p \} , \mathcal{H} \right)} \big], \mathcal{ID} \right\},
		\label{eq:quadMapPolyZono}
	\end{equation} 
	where the matrices $\overline{G}$ and $\overline{E}$ are defined as in \eqref{eq:quadMap}, $c_z$ and $G_z$ are the results from the zonotope over-approximation in \eqref{eq:quadMapZonotope} and the discrete set of indices $\mathcal{H}$ is defined as in \eqref{eq:quadMapIndices}. The complexity of the calculations is $\mathcal{O}(n^3 \log(n)) + \mathcal{O}(n^3 m)$. 
	\label{prop:quadMapSpecial}
\end{proposition} 

\begin{proof}
	(Quadratic Map) We first introduce the extended generator and exponent matrices $\hat{G}$ and $\hat{E}$ as well as the extended list of identifiers $\widehat{\mathcal{ID}}$:
	\begin{equation}
		\begin{split}
		& \hat{G} = \begin{bmatrix} G & G_I \end{bmatrix}, ~ \hat{E} = \begin{bmatrix} E & \mathbf{0} \\ \mathbf{0} & I \end{bmatrix}, \\
		& \widehat{\mathcal{ID}} = \left\{ \mathcal{ID}, M+1 , \dots, M + q \right\},
		\end{split}
		\label{eq:quadMapExtMat}
	\end{equation}
	where $I \in \mathbb{R}^{q \times q}$ is the identity matrix and $M = \max(\mathcal{ID})$. Next, we calculate $\overline{E}$ and $\overline{G}$ according to \eqref{eq:quadMap}. The resulting matrices are divided into one part that contains dependent factors only, and a second part that contains all remaining monomials using the following index sets:
	\begin{equation}
		\begin{split}
			& \mathcal{K} = \left\{ i ~\left|~ \exists j > p ~ \overline{E}_{(j,i)} \neq 0 \right. \right\}, \\
			& \mathcal{H} = \{ 1 \dots h+q \} \setminus \mathcal{K}.
			\label{eq:quadMapIndices}
		\end{split}
	\end{equation}
	Finally, the part that contains the independent factors is enclosed by a zonotope:
	\begin{equation}
		\{c_z, G_z \} = zono \left( \left\{ \overline{G}_{\left( \cdot, \mathcal{K} \right)}, \mathbf{0}, \overline{E}_{\left( \cdot, \mathcal{K} \right)}, \widehat{\mathcal{ID}} \right\} \right).
		\label{eq:quadMapZonotope}
	\end{equation} 
Since the operation $zono()$ is over-approximative, the \SPZl constructed according to \eqref{eq:quadMapPolyZono} encloses the quadratic map.

Complexity: With the extended matrices $\hat{G}$ and $\hat{E}$ from \eqref{eq:quadMapExtMat}, the calculation of $\hat{E}^{(j)}$ and $\hat{G}^{(j)}$ has complexity $\mathcal{O}((h+q)^2 (p+q))$ and $\mathcal{O}(n^2 (h+q) m) + \mathcal{O}(n (h+q)^2 m)$, respectively. Furthermore, the complexity coming from the subsequent application of the $compact()$ operation is $\mathcal{O}(ph^2 \log (h^2))$, resulting in an overall complexity of $\mathcal{O}(n^3 \log(n)) + \mathcal{O}(n^3 m)$ using \eqref{eq:complexity}.
\end{proof}
\begin{remark}
	Since the independent generators add a zonotopic part to the \SPZ, the set representing the quadratic map generally contains monomials with squared independent factors as well as monomials with products of independent factors, which can be deduced from \cite[Theorem 1]{Althoff2013a}. To represent the resulting set as a proper \SPZ, we eliminate these monomials by enclosing them with a zonotope in \eqref{eq:quadMapZonotope}, which results in an over-approximation of the quadratic map.
\end{remark}
The extension to cubic or even higher-order maps of sets is straightforward and therefore omitted due to space limitations.



% Auxiliary operations

\subsection{Auxiliary Operations}
\label{subsec:auxiliaryOperations}

% Order reduction

\paragraph{Order Reduction}

Many set operations such as Minkowski addition or quad\-ratic maps increase the number of generators, and consequently also the order $\rho$ of the \SPZ. Thus, for computational reasons, it is necessary to repeatedly reduce the zonotope order during reachability analysis. We propose a reduction operation for \SPZsl that is based on the order reduction of zonotopes (see e.g. \cite{Kopetzki2017}).

\begin{proposition}
	(Reduce) Given an \SPZl $\mathcal{PZ} = \{ G,G_I,\linebreak[1] E,\mathcal{ID} \}$ and a desired zonotope order $\rho_d$, the operation \lword{$reduce()$} returns an \SPZl with order smaller than $\rho_d$ that encloses $\mathcal{PZ}$:
	\begin{equation}
 		\begin{split}
			& reduce(\mathcal{PZ},\rho_d) = \bigg\{ \begin{bmatrix} c_z & G_{(\cdot,\widehat{\mathcal{K}})} \end{bmatrix}, \begin{bmatrix} G_{I(\cdot,\widehat{\mathcal{H}})} & G_z \end{bmatrix}, \\ 
			& ~~~~~~~~~~~~~~~~~~~~~~~~  \begin{bmatrix} \mathbf{0} & E_{(\cdot,\widehat{\mathcal{K}})} \end{bmatrix}, ~ \mathcal{ID} \bigg\} \\
			& with ~~ \{ c_z, G_z \} = reduce(\mathcal{Z},1), \\
			& ~~~~~~~~\mathcal{Z} = zono \big( \{ G_{(\cdot,\mathcal{K})},~ G_{I(\cdot,\mathcal{H})},~ E_{(\cdot,\mathcal{K})},~ \mathcal{ID} \} \big).
		\end{split}
	\end{equation}
	For reduction, we select the smallest $a = \lceil h + q - n (\rho_d-1)+1\rceil$ generators:
	\begin{equation}
	\begin{split}
		& \mathcal{K} = \left\{ i ~\left| ~ {|| G_{(\cdot,i)} ||}_2 \leq {|| \hat{G}_{(\cdot,\mathcal{N}_{(a)})} ||}_2 \right. \right\}, \\
		& \mathcal{H} = \left\{ i ~\left| ~ {|| G_{I(\cdot,i)} ||}_2 \leq {|| \hat{G}_{(\cdot,\mathcal{N}_{(a)})} ||}_2 \right. \right\},\\
		& \widehat{\mathcal{K}} = \{1, \dots ,h \} \setminus \mathcal{K},~~ \widehat{\mathcal{H}} = \{1, \dots ,q \} \setminus \mathcal{H}, \\
		& with ~~ {|| \hat{G}_{(\cdot,\mathcal{N}_{(1)})} ||}_2 \leq \dotsc \leq {||\hat{G}_{(\cdot,\mathcal{N}_{(h+q)})}||}_2~,
	\end{split}
	\label{eq:reductionIndexSets}
	\end{equation} 
	where $\hat{G} = [G~G_I]$ and $\mathcal{N} \in \{ \mathbb{Z}_{>0} \}^{h+q}$ is a discrete set of indices. The complexity is $\mathcal{O}(n^2) + \mathcal{O}(reduce())$, where $\mathcal{O}(reduce())$ denotes the complexity of the zonotope reduction, which depends on the selected method. 
\end{proposition}

\begin{proof}
	(Reduce) The definition of $a$ ensures that $|\hat{\mathcal{K}}| + |\hat{\mathcal{H}}| + n + 1 \leq \rho_d n$. Further, $reduce(\mathcal{PZ},\rho_d) \supseteq \mathcal{PZ}$ since $zono()$ and the reduction of a zonotope $reduce()$ are both over-approximative, and therefore $reduce(zono())$ is over-$\linebreak[1]$approximative, too. 
	
Complexity: Sorting the generators has a complexity of $\mathcal{O}(n(h+q)) + \mathcal{O}((h+q) \log(h+q))$, and the enclosure with a zonotope has a worst case complexity of $\mathcal{O}(ph) + \mathcal{O}(nh)$. Using \eqref{eq:complexity}, the overall complexity is therefore $\mathcal{O}(n^2) \linebreak[1] +$  \lword{$\mathcal{O}(reduce())$}.
\end{proof}
After reduction, we remove possibly generated all-zero rows in the exponent matrix.




% Restructure

\paragraph{Restructure}

Due to the repeated order reduction and Minkowski addition during reachability analysis, the volume spanned by independent generators grows relative to the volume spanned by dependent generators. As explained later in Sec. \ref{sec:ReachabilityAnalysis}, this has a negative effect on the tightness of the reachable sets. We therefore define the operation $restructure()$, which introduces new dependent generators that over-approximate the independent ones:
\begin{proposition}
	(Restructure) Given an \SPZl $\mathcal{PZ} = \{ G, \linebreak[1] G_I,E,\mathcal{ID} \}$, $restructure()$ returns an \SPZl that encloses $\mathcal{PZ}$ and removes all independent generators:
	\begin{equation}
		\begin{split}
			& restructure(\mathcal{PZ}) = \left\{\begin{bmatrix} c_z & G & G_z \end{bmatrix}, \mathbf{0}, \overline{E}, \overline{\mathcal{ID}} \right\} \\
			& with ~~ \{c_z,G_z\} = reduce(\{\mathbf{0},G_I \}, 1),~\overline{E} = \begin{bmatrix} \mathbf{0} & E & \mathbf{0} \\ \mathbf{0} & \mathbf{0} & I \end{bmatrix}, \\
			& ~~~~~~~~~ \overline{\mathcal{ID}} = \left\{ \mathcal{ID}, M+1 , \dots, M + n \right\}, ~M = \max(\mathcal{ID}),
		\end{split}
		\label{eq:restructure}
	\end{equation}
where $I \in \mathbb{R}^{n \times n}$ is the identity matrix. The overall complexity is $\mathcal{O}(reduce())$, which is the complexity of the zonotope reduction.
 \label{prop:restructure}
\end{proposition}

\begin{proof}
	The result of the $restructure()$ operation encloses the original set since $reduce()$ is over-approx\-imative, and the redefinition of independent generators as new dependent generators just changes the set representation, but not the set in \eqref{eq:restructure} itself.
	
Complexity: Since all other operations are concatenations and initializations, the complexity equals the one of $reduce()$. 
\end{proof}

We demonstrate the effectiveness of Prop. \ref{prop:restructure} by numerical examples in Sec. \ref{sec:NumericalExamples}. To save computation time, we define an upper bound $p_d$ of factors for the \SPZl after restructuring so that $p+q \leq p_d$ holds, where independent factors are removed first to maintain as much dependence as possible. 










% REACHABILITY ANALYSIS -------------------------------------

\section{Reachability Analysis}
\label{sec:ReachabilityAnalysis}

In this section we demonstrate how \SPZsl can be used to improve reachability analysis for nonlinear systems. Our algorithm is based on the conservative polynomialization approach \cite{Althoff2013a} for nonlinear systems of the form
\begin{equation}
	\dot x (t) = f(x(t),u(t)), ~ x(t) \in \mathbb{R}^n,~ u(t) \in \mathbb{R}^m,
\end{equation}
where $x$ is the vector of system states and $u$ is the input vector. The conservative polynomialization approach for reachability analysis is based on the abstraction of the nonlinear function $f(\cdot)$ by a Taylor expansion of order $\kappa$:
\begin{equation}
	\begin{split}
		\dot x_{(i)} & = f_{(i)}(z(t)) \\
		& \in \left. \sum_{j=1}^{\kappa} \frac{\left((z(t)-z^*)^T \nabla \right)^j f_{(i)}(\tilde z)}{j!} \right|_{\tilde{z} = z^*} \oplus \mathcal{L}_{(i)}(t),
	\end{split}
\end{equation} 
where the shorthand $z = [x^T~u^T]^T$ and the Nabla operator $\nabla = \sum_{i=1}^{n+m} e^{(k)} \frac{\partial}{\partial z_{(i)}}$ with $e^{(k)}$ being orthogonal unit vectors, are introduced for a concise notation. The set $\mathcal{L}_{(i)}(t)$ is the Lagrange remainder, defined in \cite[Eq. (2)]{Althoff2013a}, and the vector $z^* \in \mathbb{R}^{n+m}$ is the expansion point for the Taylor series.

\begin{algorithm}[h!tb]
	\caption{$reach(\mathcal{R}(0),t_f,\dots)$} \label{alg:reach}
	\textbf{Require:} Initial set $\mathcal{R}(0)$, input set $\mathcal{U}$, time horizon $t_f$,
	
	$~~~~~~~~~~~~~$ time step $r$, factor $\lambda$.
	
	\textbf{Ensure:} $\mathcal{R}([0,t_f])$
	\begin{algorithmic}[1]
		\State $t_0 = 0,~ s = 0,~ \mathcal{R}^{union} = \emptyset,~ \mathcal{U}^{\Delta} = \mathcal{U} \oplus (-u^c)$
		\While{$t_s < t_f$}
			\State \texttt{taylor} $\rightarrow z^*, w, A, B ,D ,E$
			\State $\Psi(\tau_s) = \mathbf{0}$
			\State $\mathcal{V}(t_s) = w \oplus B u^c \oplus \frac{1}{2}sq(D,R(t_s) \times \mathcal{U})$ \label{line:quadMap}
			\State $\mathcal{Z}_z(t_s) = zono(\mathcal{R}(t_s)) \times \mathcal{U}$
			\Repeat
				\State $\overline{\Psi} (\tau _s) = $~\texttt{enlarge}$(\Psi(\tau_s),\lambda)$ \label{line:enlarge}
				\State $\mathcal{R}_z^{\Delta}(\tau_s) = $~\texttt{post}$^{\Delta}(\mathcal{R}(t_s),\overline{\Psi} (\tau _s),A) \times \mathcal{U}$
				\State $\mathcal{R}_z^{\Delta}(\tau_s) = zono(\mathcal{R}_z^{\Delta}(\tau_s))$
				\State $\mathcal{V}^{\Delta}(\tau_s) = $~\texttt{varInputs}$(\mathcal{Z}_z(t_s),\mathcal{R}_z^{\Delta}(\tau_s),\mathcal{U}^{\Delta},B,D)$
				\State $\mathcal{R}(\tau_s) = \mathcal{R}(t_s) \oplus \mathcal{R}_z^{\Delta}(\tau_s)$
				\State $\mathcal{L}(\tau_s) = $~\texttt{lagrangeRemainder}$(\mathcal{R}(\tau_s),E,z^*)$
				\State $\Psi(\tau_s) = \mathcal{V}(t_s) \oplus \mathcal{V}^{\Delta}(\tau_s) \oplus \mathcal{L}(\tau_s)$
			\Until{$\Psi(\tau_s) \subseteq \overline{\Psi} (\tau _s)$}	
			\State $\mathcal{R}(t_{s+1}) = $~\texttt{post}$(\mathcal{R}(t_s),A,\mathcal{V}(t_s),\mathcal{V}^{\Delta}(\tau_s),\mathcal{L}(\tau_s))$ \label{line:post}
			\State $\mathcal{R}(t_{s+1}) = reduce(\mathcal{R}(t_{s+1}),\rho_d)$ \label{line:reduce}
			\If{$volRatio(\mathcal{R}(t_{s+1})) > \mu_d$}
				\State $\mathcal{R}(t_{s+1}) = restructure(\mathcal{R}(t_{s+1}))$\label{line:restructure}
			\EndIf
			\State $\mathcal{R}^{union} = \mathcal{R}^{union} \cup \mathcal{R}(\tau_s)$
			\State $t_{s+1} = t_s + r, ~ s:= s+ 1$
		\EndWhile
		\State $\mathcal{R}([0,t_f]) = \mathcal{R}^{union}$
	\end{algorithmic}
\end{algorithm}


In order to fully exploit the advantages of \SPZs, Alg. \ref{alg:reach} is slightly modified from \cite{Althoff2013a}. We only specify the algorithm for the Taylor order $\kappa = 2$ for simplicity, since the extension to higher orders is straightforward. The definitions of the operators \texttt{taylor}, \texttt{enlarge}, \texttt{post}$^{\Delta}$, \texttt{varInputs}, and \texttt{lagrangeRemainder} are identical to the ones in \cite{Althoff2013a}. Only the definition of the \texttt{post} operator changed, since we precompute some of the sets in our algorithm: 

\begin{equation}
	\begin{split}
		& \mathrm{\texttt{post}}\left(\mathcal{R}(t_s),A,\mathcal{V}(t_s),\mathcal{V}^{\Delta}(\tau_s),\mathcal{L}(\tau_s)\right) = \\
		& ~~~ \underbrace{e^{Ar} \mathcal{R}(t_s)}_{\mathcal{F}_1} \oplus \underbrace{\Gamma(r) \mathcal{V}(t_s)}_{\mathcal{F}_2} \oplus \mathcal{R}^{p,\Delta}\left(\mathcal{V}^{\Delta}(\tau_s) \oplus \mathcal{L}(\tau_s),r\right),
	\end{split}
	\label{eq:post}
\end{equation}
where $\mathcal{R}^{p,\Delta}(\cdot)$ is defined as in \cite[Eq. (9)]{Althoff2013a}, and the definition for $\Gamma(r)$ can be found in \cite[Sec. 3.2]{Althoff2013a}. We proceed with a discussion of the main advantages resulting from using \SPZs.



% Advantages Sparse Polynomial Zonotopes

\subsection{Advantages of using Sparse Polynomial Zonotopes}

\label{subsec:advantages}

As mentioned earlier, one of the main advantages of \SPZsl is that they reduce the dependency problem in Alg. \ref{alg:reach}. We demonstrate this with a short example: 

\begin{example}
Consider a one-dimensional problem without inputs: a reachable set $\mathcal{R}(t_s) = \{\alpha_1 | \alpha_1 \in [-1,1] \}$, the parameter values $w=0$, $A=1$, $D=2$, and $r=1$. The quadratic map in line \ref{line:quadMap} of Alg. \ref{alg:reach} evaluates to $\frac{1}{2} sq(D,\mathcal{R}(t_s)) = \{\alpha_1^2 | \alpha_1 \in [-1,1] \}$ for \SPZs. On the other hand, if we use zonotopes, then the quadratic map has to be over-approximated with $\frac{1}{2} sq(D,\mathcal{R}(t_s)) = \{0.5 + 0.5 \alpha_2 | \alpha_2 \in [-1,1] \}$. With zonotopes, we therefore obtain for \eqref{eq:post}
\begin{equation}
	\begin{split}
		\mathcal{F}_1 \oplus \mathcal{F}_2 = \big \{ & 2.718 \alpha_1 + 1.718(0.5 + 0.5 \alpha_2)   \\
		& |~ \alpha_1,\alpha_2 \in [-1,1] \big \} = [-2.718,4.436].
		\end{split}
\end{equation}
With \SPZs, however, we obtain the exact set
\begin{equation}
	\begin{split}
		\mathcal{F}_1 \oplus \mathcal{F}_2 = \big \{ & 2.718 \alpha_1 + 1.718 \alpha_1^2 ~|~ \alpha_1 \in [-1,1] \big \} \\
		& = [-1.075,4.436].
		\end{split}
\end{equation}
\end{example}
Using zonotopes for reachability analysis therefore leads to a significant over-approximation error in each time step. A similar problem occurs with the polynomial zonotope representation from \cite{Althoff2013a}, since this requires limiting the maximum polynomial degree in advance.  

With our new \SPZl representation, it is in theory even possible to approximate the exact reachable set arbitrarily close: 
\begin{theorem}
	Let us consider the case without uncertain inputs $\mathcal{U} = \emptyset$, with parameter values $\rho_d = \infty$, $\mu_d = 0$, and $f(\cdot)$ being a $C^{\infty}$ differentiable function. In addition, $\kappa$ is chosen large enough to ensure that $\mathcal{L}(\tau_s) \rightarrow \mathbf{0}$. We further assume that the enlargement factor $\lambda$ in line \ref{line:enlarge} of Alg. \ref{alg:reach} is always chosen such that $\Psi(\tau_s) = \overline{\Psi}(\tau_s)$ holds, and that the $restructure()$ operation does not result in an over-approximation, which can easily be achieved by omitting the reduction step. The reachable set computed with \SPZsl would then converge to the exact reachable set for $r \rightarrow 0$.
\end{theorem}

\begin{proof} 
If $\mu_d = 0$, we execute the $restructure()$ operation in every time step. The set $\mathcal{R}(t_s)$ is therefore an \SPZl without independent generators, which implies that the quad\-ratic map does not result in an over-approximation. Consequently, the only operation that leads to an over-appro\-ximation is the Minkowski addition of the set $\mathcal{R}^{p,\Delta}(\cdot)$ during the evaluation of the \texttt{post} operator as shown in \eqref{eq:post}. This over-approximation error converges to zero for $r \rightarrow 0$, since per definition $\mathcal{R}^{\Delta}(\tau_s) \rightarrow \mathbf{0}$ for $r \rightarrow 0$ \cite[Eq. (6)]{Althoff2013a}, and therefore $\mathcal{R}^{p,\Delta}(\cdot) \rightarrow \mathbf{0}$ for $r \rightarrow 0$.
\end{proof}




% Hybrid systems

\subsection{Hybrid Systems}

In reachability analysis for hybrid systems, the main difficulty is the calculation of the intersection between the reachable set and the guard sets. Since it is in general computationally infeasible to calculate this intersection directly for \SPZs, we propose calculating the intersection with a zonotope over-approximation instead. By doing so it is possible to directly apply the well-developed techniques for the computation of guard intersections with zonotopes, like e.g., the ones from \cite{Girard2008} or \cite{Althoff2012a}. Note that even if the intersections with the guard sets are calculated with a zonotope over-approximation, the reachable set of the hybrid system calculated with \SPZsl is generally much tighter than the one calculated with zonotopes (see Sec. \ref{sec:NumericalExamples}).






% NUMERICAL EXAMPLES  ---------------------------------------

\section{Numerical Examples}
\label{sec:NumericalExamples}

In this section we demonstrate the improvements to reachability analysis due to using \SPZsl on two benchmark systems. All computations are carried out in MATLAB on a 2.9GHz quad-core i7 processor with 32GB memory. We heuristically trigger the restructure process (see Sec. \ref{subsec:auxiliaryOperations}) when $volRatio(\mathcal{PZ}) = \frac{vol(interval(\{ \mathbf{0}, G_I \}))}{vol(interval(zono(\{G,\mathbf{0},E,\mathcal{ID} \})))} > \mu_d$, where $\mathcal{PZ} = \{ G, G_I,E,\mathcal{ID} \}$ and $vol(\cdot)$ calculates the volume of a multi-dimensional interval. 

\begin{figure}
\begin{center}
	\setlength{\belowcaptionskip}{-20pt}
	\includegraphics[width = 0.48 \textwidth]{figures/VanDerPol.pdf}
	\caption{Reachable set of the Van-Der-Pol oscillator calculated with different set representations.}
	\label{fig:vanDerPol}
	\end{center}
\end{figure}

The system considered first is the Van-der-Pol oscillator taken from the 2018 ARCH competition \cite{ARCH18nonlinear}:

\begin{equation}
	\begin{split}
		& \dot x_1 = x_2 \\
		& \dot x_2 = (1-x_1^2) x_2 - x_1.
	\end{split}
\end{equation} 
For this system, we compare the results for the computation of the reachable set with Alg. \ref{alg:reach} using zonotopes, the quadratic zonotopes from \cite{Althoff2013a} and our \SPZl representation. We consider the initial set $x_1 \in [1.23,1.57]$ and $x_2 \in [2.34,2.46]$, and use a time step size of $r = 0.005$ seconds, a maximum zonotope order of $p_d = 50$, an enlargement factor of $\lambda = 0.1$, a maximum volume ratio of $\mu_d = 0.01$, and an upper bound for the number of dependent factors of $p_d = 100$. The method in \cite[Sec. 3.4]{Girard2005} (Girard's method) is applied for zonotope reduction, and we use principal-component-analysis-based order reduction in combination with the Girard's method for the reduction during the restructure operation (see \cite{Kopetzki2017}). For a fair comparison, we use the same parameter values for every set representation. 

The resulting reachable sets are shown in Fig. \ref{fig:vanDerPol}. It is clearly visible that the stability of the limit cycle can only be verified with \SPZsl when sets are not split. The computation time is $9.33$ seconds for linear zonotopes, $13.38$ seconds for quadratic zonotopes, and $16.52$ seconds for \SPZs.

\begin{figure}[h]
\begin{center}
	\setlength{\belowcaptionskip}{-20pt}
	\includegraphics[width = 0.48 \textwidth]{figures/VanDerPolSingleSet.pdf}
	\caption{Comparison of the real reachable set of the Van-Der-Pol oscillator after $\mathbf{t=3.15~seconds}$ with the reachable set over-approximation calculated with \SPZs.}
	\label{fig:vanDerPolSingleSet}
	\end{center}
\end{figure}

An impression on how tight the reachable set can be over-approximated with \SPZsl is provided in Fig. \ref{fig:vanDerPolSingleSet}, where the reachable set after $t = 3.15$ seconds computed with a time step size of $r = 0.0001$ seconds and a maximum volume ratio of $\mu_d = 0.001$ is compared to the exact reachable set of the system. The figure also demonstrates how well the \SPZl approximates the shape of the exact reachable set. 

For the second numerical example, we examine a drive\-train \cite{Lagerberg2007}, which is a benchmark from the ARCH 2018 competition \cite{ARCH18linear}, too. We consider the case with $2$ rotating masses, resulting in a system dimension of $n=11$. The model is a hybrid system with linear dynamics. However, we apply the novel approach from \cite{Bak2017c} for calculating the intersections with guard sets, which is based on time-triggered conversion of guards and results in a significant nonlinearity due to the time scaling process. The initial set is given by $\mathcal{R}_0 = 0.5 (\mathcal{X}_0 - center(\mathcal{X}_0)) + center(\mathcal{X}_0)$, where $\mathcal{X}_0$ is defined as in \cite{ARCH18linear}, and we consider the same extreme acceleration maneuver as in \cite{ARCH18linear}. As a specification, we require that the engine torque after $1.5$ seconds is at least $59 Nm$, which can formally be specified as $T_m \geq 59Nm ~ \forall t \geq 1.5 s$. 

\begin{figure}[h]
\begin{center}
	\setlength{\belowcaptionskip}{-10pt}
	\includegraphics[width = 0.48 \textwidth]{figures/Drivetrain.pdf}
	\caption{Reachable sets for the drivetrain benchmark calculated with zonotopes (left), quadratic zonotopes (middle), and \SPZsl (right). The forbidden set defined by the specification is depicted in orange.}
	\label{fig:drivetrain}
	\end{center}
\end{figure}

The results for the drivetrain model are shown in Fig. \ref{fig:drivetrain}. We explicitly considered the possibility of splitting the reachable sets, so that the specification could be verified with all set representations. However, splitting sets prolongs the computation time: with quadratic zonotopes, the verification took $93$ seconds, and $221$ seconds with zonotopes. Only with \SPZsl it was possible to verify the specification without splitting, resulting in a computation time of $15$ seconds, which is $6$ times faster than with quadratic zonotopes and more than $14$ times faster than with zonotopes. Compared to other non-zonotopic set representations, the speed-up is even larger: in the results for this benchmark from the ARCH 18 competition \cite{ARCH18linear}, the tool \textit{CORA}, which uses zonotopes to represent reachable sets, had for the high dimensional test cases with large initial set the smallest computation time compared to the other participating tools \textit{Flow*} and \textit{Hylaa}, which use Taylor models and star sets, respectively.






% CONCLUSIONS ---------------------------------------------

\section{Conclusions}

We have introduced \textit{sparse polynomial zonotopes}, a new non-convex set representation. The sparsity results in several advantages compared to previous representations of polynomial zonotopes: sparse polynomial zonotopes enable a compact representation of sets, they are closed under all relevant set operations, and all operations have at most polynomial complexity. The fact that sparse polynomial zonotopes include several other set representations like Taylor models and zonotopes further substantiates the relevance of the new representation.

One application for sparse polynomial zonotopes is reachability analysis for nonlinear systems. Our improved reachability algorithm exploits the advantages of sparse polynomial zonotopes. The numerical examples demonstrate that our approach indeed computes much tighter over-approximations of reachable sets compared to zonotopes and quadratic zonotopes. Due to the improved accuracy, splitting can be avoided by using sparse polynomial zonotopes, which results in a significant reduction of the computation time since the complexity of splitting sets grows exponentially with the system dimension.
